A HARPS radial velocity search for planets in the Scorpius-Centaurus association. And its combination with the HARPS and SOPHIE young nearby stars (YNS) surveys

The Scorpius-Centaurus (Sco-Cen) young and nearby massive star-forming region is particularly well suited for extrasolar planet searches with both direct imaging and radial velocity (RV) techniques. The RV search, however, is challenging, as the stars are faster rotators on average than their older stellar counterparts of similar spectral types. Moreover, the RV time series show strong signatures of stellar variability (spots and faculae) and/or stellar pulsations. Our aim is to search for giant planets (GPs) and brown dwarfs at short orbital distances around star members of the Sco-Cen association. We also aim at using these data together with others available on young stars to estimate the GP occurrence rate for young stars for periods of up to 1000 days. We used the HARPS spectrograph on the 3.6m telescope at the La Silla Observatory to monitor 88 A-F Sco-Cen stars. To improve our statistics and analysis, we combined this survey with two previous surveys that focused on young nearby stars (YNS) to compute companion occurrence rates from a sample of 176 young A-M stars. We report the discovery of a massive hot-Jupiter candidate around HD 145467, together with the discovery of one probable short-period (P < 10 days) brown dwarf around HD 149790. In addition, we confirm the binary nature of eight single-line binaries: HD 108857, HD 108904, HD 111102, HD 114319, HD 121176, HD 126488, HD 126838, and HD 133574. From our sample, we obtain a GP ($m_c\in[1;13] M_{Jup}$) occurrence rate of $0.7_{-0.2}^{+1.6} \ \%$ for periods between 1 and 1000 days and a brown dwarf ($m_c\in[13;80] M_{Jup}$) occurrence rate of $0.6_{-0.2}^{+1.4} \ \%$, in the same period range. In addition, we report a possible lack of close ($P\in[1;1000] days$) GPs around young F-K stars compared to their older counterparts, with a confidence level of 95%.

==> abstract <==
Context : The young and nearby massive star forming region of Scorpius-Centaurus (Sco-Cen) is particularly well suited for extrasolar planet searches, being the target of both direct imaging and radial velocity (RV) surveys. The RV study of such young stars can be particularly challenging, as they are on average faster rotators than their older stellar counterparts of similar spectral type. In general, they induce much stronger signatures of stellar variability (spots and faculae) and/or stellar pulsations into their RV time series. In order to analyse the data and search for planets, it is required to take these nuisance signals into account and correct for them.
Aim : Our aim is to search for short separations planets around Sco-Cen stars and to estimate the giant planets (GPs) occurrence rates for periods of up to 1000 days.
Method : We used the HARPS  spectrograph on the \3.6m telescope at La Silla Observatory to monitor 89 A-F Sco-Cen stars. To compute the RVs and other spectroscopic observables we applied our SAFIR (Spectroscopic data via Analysis of the Fourier Interspectrum Radial velocities) software. To improve our statistics and analysis we combined this survey with the HARPS young nearby stars (YNS) survey and the SOPHIE YNS survey, allowing us to compute companion occurrence rates on a total of 177 young A-M stars.
Result : We report the discovery of  a hot Jupiter candidate, that needs to be confirmed,  around HD 145467, together with the discovery of one probable short period (P<10 days) brown dwarf around HD 149790.
In addition, we report the discovery of 3 double lined binaries: HD 129590, HD 137057, HD 143811 and we confirm the binary nature  of 8 single lined binaries: HD 108857, HD 108904, HD 111102, HD 114319, HD 121176, HD 126488, HD 126838, and HD 133574.  Based on our 177 young stars sample, we obtain a GPs (1 < m_c < 13 MJ) occurrence rate of  0.7_-0.2^+1.6 % for periods between 1 and  1000 days and a brown dwarf (13 < m_c < 80 MJ) occurrence rate  of 0.6_-0.2^+1.4 %,  in the same period range. In addition, we report a possible lack of close (1 < P < 1000 days GPs around young F-K stars compared to their older counterparts, with a confidence level of 95%.

ref number : AA/2021/41235
